AIpparel: A Multimodal Foundation Model for Digital Garments

Apparel is essential to human life, offering protection, mirroring cultural identities, and showcasing personal style. Yet, the creation of garments remains a time-consuming process, largely due to the manual work involved in designing them. To simplify this process, we introduce AIpparel, a multimodal foundation model for generating and editing sewing patterns. Our model fine-tunes state-of-the-art large multimodal models (LMMs) on a custom-curated large-scale dataset of over 120,000 unique garments, each with multimodal annotations including text, images, and sewing patterns. Additionally, we propose a novel tokenization scheme that concisely encodes these complex sewing patterns so that LLMs can learn to predict them efficiently. AIpparel achieves state-of-the-art performance in single-modal tasks, including text-to-garment and image-to-garment prediction, and enables novel multimodal garment generation applications such as interactive garment editing. The project website is at https://georgenakayama.github.io/AIpparel/.

==> sec/1_intro.tex <==
\section*{Introduction}
\label{sec:intro}

%-------------------------------------------------------------------------

% Clothing is essential to human life, offering protection, mirroring cultural identities, and showcasing personal style.
Apparel plays a crucial role in society, serving as a barrier against the elements, a reflection of societal norms, and a means of personal expression. 
A key stage in garment production is the development of sewing patterns---a set of flat 2D panels with standardized assembly instructions that form a complete 3D garment~\citep{Armstrong:2009}.
%~\cite{liu2023sewformer, clo3d}.
% Pattern making is a time-consuming and challenging task because sewing patterns often involve complex geometry, requiring even experienced tailors to undergo multiple iterations, incorporating feedback from different modalities, including language descriptions of fit and feel of the garment and visual references of its appearance. 
Pattern making is a challenging task due to the complex geometric relationship between the sewing pattern and the draped garment in 3D. 
Even an experienced tailor must go through multiple iterations, incorporating feedback from various sources, including verbal descriptions of the garment's fit and feel, as well as visual references of its appearance. 
% because sewing patterns often involve complex geometry, requiring even experienced tailors to undergo multiple iterations, incorporating feedback from different modalities, including language descriptions of fit and feel of the garment and visual references of its appearance. 
%In this paper, we explore the question: can we develop algorithms to predict and generate sewing patterns from different modalities?
To simplify the pattern-making process, we explore strategies to leverage emerging generative models with multimodal inputs, such as language and images.
% how one can learn to generate sewing patterns from 
% using large multimodal generative models.

State-of-the-art sewing pattern prediction methods are designed to work with one specific input modality, such as 3D points~\cite{NeuralTailor2022,bang2021estimating,chen2015_garment_modeling_w_depth}, images~\cite{pietroni2022computational,yunchu2007prototype,wolff20213d,nariatposeindependent,yang2016detailedgarmentrecoverysingleview}, or language~\cite{he2024dresscodeautoregressivelysewinggenerating}.
While effective within their domains, adapting them for garment prediction from multiple input modalities remains difficult mainly for two reasons. 
% Expanding these methods to multimodal pattern prediction presents two primary challenges. 
First, no large-scale sewing pattern dataset with multimodal annotation is publicly available, limiting the data-driven methods' generalizability. 
Second, the existing methods are capacity-limited for multimodal generation, since the ability to accurately interpret multimodal inputs typically only emerges in large models with billions of parameters~\cite{achiam2023gpt,liu2023llava}. 
% It remains uncertain how to efficiently scale existing methods to models of this size.
% Current multimodal garment prediction efforts generally focus only on generating garment images~\cite{baldrati2023multimodal,jiang2022text2human}. 
% Converting these images into sewing patterns typically involves an additional stage operating independently of the original multimodal input, which can be error-prone.
% Prior methods capable of generating sewing patterns from multimodal inputs, such as \citet{Wang2018LearningAS}, are usually restricted to garments with a predefined set of parameters, limiting their applicability to garments with complex geometries.

% Rather than training specialized models from scratch for pattern prediction from a single modality, we
This paper proposes ways to tackle both of these obstacles.
To address the lack of multimodal annotations, we present GarmentCodeData-MultiModal (GCD-MM), an extension to the largest publically available sewing pattern dataset~\cite{korosteleva2024garmentcodedatadataset3dmadetomeasure} to multimodal annotations. GCD-MM is ten times larger than those used by previous state-of-the-art generative methods~\cite{NeuralTailor2022, liu2023sewformer, he2024dresscodeautoregressivelysewinggenerating}, including over 120,000 unique sewing patterns paired with detailed text descriptions, images, edited sewing patterns, and editing instructions. 
We propose to address the limited model capacity by fine-tuning existing large multimodal models (LMMs)~\cite{gpt4tools, touvron2023llama2openfoundation, liu2023llava} to understand sewing patterns with complex geometries.
% It allows our model to generate a diverse set of sewing patterns conditioned on different categories of inputs.   
% To achieve this, we annotate the largest sewing pattern dataset \cite{korosteleva2024garmentcodedatadataset3dmadetomeasure} with multimodal labels. 
% Fine-tuning an LMM to perform multimodal garment generation requires representing complex garments in a format existing LMMs can understand.
To achieve this, we propose a novel sewing pattern tokenization scheme and a fine-tuning objective that is both expressive enough to represent the complex and diverse geometries of sewing patterns and compact enough to fit within the limited context length of existing LMMs, making fine-tuning computationally efficient. 

Combining these components, we present \textbf{\methodname}, a large multimodal model for generating sewing patterns.
\methodname can predict sewing patterns with complex geometry and outperform state-of-the-art methods in single-modal garment prediction, often by a large margin. Moreover, \methodname unlocks entirely new tasks such as multimodal garment generation language-instructed garment editing.
% More importantly, \methodname unlocks multimodal sewing pattern tasks that were previously not possible, \todo{such as language-driven editing of complex garments.}
% and multimodal garment understanding.
In summary, our contributions are as follows:
\begin{itemize}
\item We present GCD-MM, a multimodal sewing pattern dataset extending the largest, public dataset with multimodal annotations.
% We curate the first multimodal sewing pattern dataset of 120,000 unique sewing patterns, each paired with rich multimodal annotations. 
We plan to release the dataset to enable research in multimodal garment generation.
\item We propose a novel tokenization scheme and training objective for fine-tuning LMMs to predict sewing patterns. 
These technical contributions are critical to retargeting LMMs to multimodal garment prediction tasks efficiently.
\item Our model, \methodname, is the first large multimodal generative model for sewing pattern prediction capable of taking language, images, and sewing patterns as input. 
We will publish the code and model.
% To the best of our knowledge, 
% \methodname is the first model capable of generating and editing garments based on multimodal inputs, including natural language and images. 
\end{itemize}

% \todo{talk about dataset statistics: we have amassed more than 120,000 garments with more than XXX tokens of language and XXX images. This is the the first and the largest multimodal garment dataset so far.}

% by fine-tuning LLMs on multimodal garment data. We showcases that using our method we can extract VLMs' general reasoning ability to garment understanding. 

% One of the fundamental challenges in developing a generative model for sewing patterns is the scarcity of large-scale public domain data with multimodal annotations. 

% context
% \todo{Need to change this paragraph to focus on motivation.}

% These unprecedented capabilities can improve the productivity of fashion designers or enable anyone to create their own designs. 

% With the advance of generative AI, digital garment design is becoming increasingly popular and is at the core of many industries such as digital avatars~\cite{PhysAavatar24}, virtual try-ons~\cite{yang2024texturepreserving}, and fabrication~\cite{mitra2024singular}. 

% and fine-tune VLMs on a combination of input modalities with new vocabularies designated to representing sewing patterns. 
% We hope that this can transfer their world-level knowledge to garment reasoning with complex inputs suitable for the garment designing process. However, while studies have investigated the generalizability of LLMs to reasoning about human poses~\cite{feng2024chatpose}, segmentation~\cite{lai2023lisa}, and robotic action planning~\cite{rt22023arxiv}, garment prediction is inherently a more complex task~\cite{liu2023sewformer} as it requires predicting both continuous parameters such as the placement of vertices and discrete parameters such as the connectivities of panels. This leads us to ask if LLMs can exhibit similar reasoning capability for garments. 


% enables a transform the field of garment design, by enabling iterative, multi-modal garment generation. Furtheremore, our experiments with semi-automatic data captioning and garment tokenization can be independently applied to other fields, where current data scarcity is a bottleneck for foundation level training. While our generated garments cover a large part of current designs, our foundation model is unable to generate accessories, such as pockets or buttons. The exensibility of our model through it transformer-based architecture lends itself to future work with even more realisitic garment design. 

% Based on newly available datasets \cite{KorostelevaGarmentData,liu2023towards, korosteleva2024garmentcodedatadataset3dmadetomeasure}, curate a large pooled dataset of multi-modal garment data. Using rule-based methods, we create high quality text descriptions for each individual garment and expand on these using pre-trained LLMs  \cite{openai2024gpt4technicalreport}. We develop an optimal tokenizable representation for garments that allows pre-trained models to quickly learn the structure of garments. The benefits of this are that our representation is more compact (by 40\% compared the SOTA \cite{he2024dresscodeautoregressivelysewinggenerating}) and more natural for transformer-based architecture to understand. We then fine-tune an existing multi-modal foundation model using our curated dataet and unique representation. This allows us to complete tasks using one model instead of multiple task based models. 

% Unfortunately, the process for garment design has remained the same as well. While occasionally incorperating ditigal tools instead of pen and paper, the iterative process of garment design remains labor intensive and time consuming \cite{clo3d}. Throughout the last years, foundational models have revolutionized the fields of natural language processing, machine translation and computer vision \cite{openai2024gpt4technicalreport,vaswani2023attentionneed,peebles2023scalablediffusionmodelstransformers}. With our work, we aim to use the principles of foundation models to transform the field of garment generation. 

% \subsection{Problem Statement}
% Foundation models minimize inductive biases and are able to generalize to a wide range of tasks \cite{openai2024gpt4technicalreport}. Although this is a really successfull principle, it necessitates a large amount of data to train on. This is a problem for garment generation, as the amount of multi-modal, accurately labelled data with high quality sewing patterns is limited. Current attempts at generating or reconstructing garments therefore stick to specialized models trained for single modal tasks \cite{NeuralTailor2022,liu2023towards,he2024dresscodeautoregressivelysewinggenerating}. Although this is works for each task in itself, it is not scalable to mutli-modal, interactive and iterative garment design. 

% \subsection{Proposed Approach}
% In this paper, we propose a new approach, called Garment Foundation Model. Based on newly available datasets \cite{KorostelevaGarmentData,liu2023towards, korosteleva2024garmentcodedatadataset3dmadetomeasure}, curate a large pooled dataset of multi-modal garment data. Using rule-based methods, we create high quality text descriptions for each individual garment and expand on these using pre-trained LLMs  \cite{openai2024gpt4technicalreport}. We develop an optimal tokenizable representation for garments that allows pre-trained models to quickly learn the structure of garments. The benefits of this are that our representation is more compact (by 40\% compared the SOTA \cite{he2024dresscodeautoregressivelysewinggenerating}) and more natural for transformer-based architecture to understand. We then fine-tune an existing multi-modal foundation model using our curated dataet and unique representation. This allows us to complete tasks using one model instead of multiple task based models. 

% \subsection{Impact}
% Our approach enables us to transform the field of garment design, by enabling iterative, multi-modal garment generation. Furtheremore, our experiments with semi-automatic data captioning and garment tokenization can be independently applied to other fields, where current data scarcity is a bottleneck for foundation level training. While our generated garments cover a large part of current designs, our foundation model is unable to generate accessories, such as pockets or buttons. The exensibility of our model through it transformer-based architecture lends itself to future work with even more realisitic garment design. 


% \subsection{Contributions}
% Here is a quick summary of our paper. In particular, we make the following contributions:
% \begin{itemize}
%   \item We introduce a garment foundation model as a new way of approaching the iterative design process of garments. 
%   \item We develop new captioning systerm for garments and a learning based representation that is more compact and natural for transformer-based models to understand.
%   \item We analyze our approach and show that it is able to handle different modalities, able to iterate over previous inputs and generate higher quality garments than the current state of the art. 
%   \item We evaluate our approach using custom quantiative and qualitative metrics. 
% \end{itemize}




% Why is it important now, why not three years ago 
% Has not been to garment geenration yet, novel approach 
% One strong, do not mix a bunch of things up front. 
% Writing paper is oversimplification of what we do \newline \newline
% Set the siginificance of the thing you are doing, reviewers need to see that it is important \newline
% For first paragraph: 
% \begin{enumerate}
%   \item if small improvement for something that everyone thinks is important, will be in itself important and interesting to many people 
%   \item garment themselves are important (make that argument), garment generaiton in itself is small field 
%   \item Need to pick one problem, problem statement (collection of problems could also be useful)
% \end{enumerate}
% Th\newline \newline 
% Second paragraph: how is it done today: 
% \begin{itemize}
%   \item Probelm with method A, B, C 
%   \item first lsit them 
%   \item Fast forward of related work section
% \end{itemize}
% THird paragraph: What our methods is: 
% \begin{itemize}
%   \item Do not address somethign that you cannot solve 
%   \item Overclaim something, that you cannot deliver 
%   \item Do not use words like 'revolutionize', 'transformative'
% \end{itemize}
% Last paragraph:
% \begin{itemize}
%   \item Contributions, best to do in bullet points as well
%   \item You want to specify what these contributions are (3-5 contributions), introduce new idea, introduce prototype, 
%   \item one section per contribtion
% \end{itemize}


% Such pattern-making is typically performed by skilled industry experts and involves iterative adjustments based on diverse inputs such as language instructions, sketches, and a combination of visual and verbal inputs.

% More recently, combining machine learning with garment design has enabled garment recovery and prediction from ambiguous inputs such as images~\cite{liu2023sewformer}, texts~\cite{he2024dresscodeautoregressivelysewinggenerating}, and point clouds~\cite{NeuralTailor2022}. While aiming to transform the classical garment design with artificial intelligence, these methods still have limited practicality as they are restricted to garment prediction given a single modality, whereas garment design often requires an iterative process with the designers giving garment specifications in a diverse set of inputs. 

% \george{Might also be good to include here that single modal prediction is also inherently ambiguous and unnatural in the context of the designing process}
% problem statement
% In this project, we aim to develop a virtual garment design assistant that can intelligently reason with garments to capture the complex interplay of common-sense physics, geometry, and the designer’s intentions. Furthermore, because the design process often involves iterative instructions in different modalities (e.g., text descriptions and sketches), virtual assistants should be capable of predicting garments given a combination of \george{not sure yet: texts, images, and point-clouds} as well as making reasonable edits on existing garments based on textual or visual guidance. 


% Garments are crucial to humanity, providing essential functions like protection while reflecting cultural identity and expressing personality. 
% Yet, the fashion industry today is dominated by prêt-à-porter (\ie, ready-to-wear) garments that grossly approximate individual body measurements and preferences and limited creativity. 
% Bespoke tailoring provides an alternative, albeit at a high cost, which is not affordable by most and requires highly skilled fashion designers and tailors. 
% Although emerging generative AI technologies, such as text-to-image and text-to-video models, can create fashion sketches or try-on videos~\cite{shen2024imagdressingv1customizablevirtualdressing,fang2024vivid}, creating fabricable garments still requires converting images or videos into sewing patterns - collections of flat 2D panels along with standardized instructions to assemble them into a garment~\cite{liu2023sewformer, clo3d}. 
% This pattern-making process remains time-consuming and requires years of training. 
% Can we develop algorithms to facilitate and automate this pattern-making process, making bespoke tailoring accessible to everyone?

% Heuristic-based approaches, however, are limited in their ability to understand complex signals, such as natural language.
% Recently, supervised deep learning methods have been developed to predict sewing patterns from a specific type of input, such as text~\cite{he2024dresscodeautoregressivelysewinggenerating}, images~\cite{liu2023sewformer}, or point clouds~\cite{NeuralTailor2022}.


==> tables/image2garment_sewfactory.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{lcccccc}
    \toprule
         Method &  Panel L2 $(\downarrow)$ & \#Panel Acc $(\uparrow)$ & Edge Acc $(\uparrow)$  & Rot L2 $(\downarrow)$ & Transl L2 $(\downarrow)$ & Stitch Acc $(\uparrow)$\\\midrule
    % SewFormer pretrained & & & & && \\    
    % DressCode pretrained (+ GPT4V)  & & & & &&\\
    % Sewformer-pretrained \\
    SewFormer & 3.34 & 89.8 & 99.3 & 0.00782 & 0.824 & 99.1\\
    % DressCode-FT (+ our caption)  & & & & &&\\
    % \midrule
      % LLaVA (in-context)   & & & & &&\\
      % GPT4V (in-context)   & & & & &&\\
    % \midrule 
      \methodname   & \textbf{2.83} & \textbf{919} & \textbf{99.9} & \textbf{0.0054} & \textbf{0.795} & \todo{98.9} \\
    \bottomrule
    \end{tabular}
    \vspace{-1em}
    \caption{\textbf{Image to Garment.} We report the garment reconstruction metrics of both Sewformer and our model in \todo{GarmentCode~\cite{TODO} dataset, which contains complex and real-world garments}. Our model achieves better performance in all metrics.\todo{On Sewformer's dataset itself?}}
    \label{tab:image2garment}
\end{table*}

==> tables/pattern_completion.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lccc}
    \toprule
    Method &  Panel L2 & \#Panel Acc & \#Edge Acc \\\midrule
      DressCode   & \\
      Ours - Mixed Obj. &\\
      Ours   & \\
      \bottomrule
    \end{tabular}
    \caption{\textbf{Tokenization Comparison on Pattern Completion}}
    \label{tab:pattern_completion}
\end{table}
